Adaptive Testing for High-dimensional Data

In this article, we propose a class of $L_q$-norm based U-statistics for a family of global testing problems related to high-dimensional data. This includes testing of mean vector and its spatial sign, simultaneous testing of linear model coefficients, and testing of component-wise independence for high-dimensional observations, among others. Under the null hypothesis, we derive asymptotic normality and independence between $L_q$-norm based U-statistics for several $q$s under mild moment and cumulant conditions. A simple combination of two studentized $L_q$-based test statistics via their $p$-values is proposed and is shown to attain great power against alternatives of different sparsity. Our work is a substantial extension of He et al. (2021), which is mostly focused on mean and covariance testing, and we manage to provide a general treatment of asymptotic independence of $L_q$-norm based U-statistics for a wide class of kernels. To alleviate the computation burden, we introduce a variant of the proposed U-statistics by using the monotone indices in the summation, resulting in a U-statistic with asymmetric kernel. A dynamic programming method is introduced to reduce the computational cost from $O(n^{qr})$, which is required for the calculation of the full U-statistic, to $O(n^r)$ where $r$ is the order of the kernel. Numerical studies further corroborate the advantage of the proposed adaptive test as compared to some existing competitors.

==> unused <==
\subsection{Testing Linear Model Coefficients}
This section includes the simulations for testing linear regression coefficients. We test $\bbeta=\bm{0}$ against $\bbeta\not=\bm{0}$. Recall the kernel function is of order 2,
$$
h_l(W_1,W_2)=[(X_1-X_2)(Y_1-Y_2-(X_1-X_2)^T\bbeta_0)]_l/2,$$
and the parameter to test equals $\|\Sigma \bbeta\|_q^q=\|\bbeta\|_q^q$ (recall here the norms are defined without taking the absolute values).

%%We use the permutation based method to simulate the null distribution introduced in Section 5.4. We randomly permute the pairings between $X_i$ and $Y_i$, and estimate the variance based on the statistics calculated from $B=10,100$ permutations. For $B=100$, we also compare the variance estimator based on permutation with the purely permutation based test. We run 1000 MC repetitions for the size simulation, and 100 ones for power simulation. We take $(n,p)=(200,100),(400,200)$, $\bbeta=\delta (\bm{1}_r,\bm{0}_{p-r}),\Sigma=I_p$ and consider $q=1,2,3,4$.  
The following results are based on MC variance.
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
$(n,p)$ & $\delta,r$ & $q=1$ & $q=2$ & $q=3$ & $q=4$ & $q=5$ & $q=6$ \\ \hline
\multirow{4}{*}{(200, 100)} & 0, NA & 5.8 & 7.8 & 6.5 & 6.9 & 5.9 & 5.8 \\ \cline{2-8}
& 2,0.2 & 9 & 22 & 33 & 41 & 36 & 29 \\ \cline{2-8}
& 2,0.4 & 22 & 76 & 95 & 98 & 96 & 95 \\ \cline{2-8}
& $0.1,p$  & 100 & 99 & 69 & 37 & 31 & 29  \\ \hline

\multirow{2}{*}{(400, 200)} & 2,0.2 & 11 & 32 & 58 & 77 & 75 & 69 \\ \cline{2-8}
& $0.1,p$  & 100 & 100 & 98 & 67 & 37 & 25  \\ \hline

\end{tabular}
\caption{Size and power simulation in \%, with variance estimator based on permutation}
\end{table}
Since the expectation of the U-statistics equals $\|\bbeta\|_q$ with our specific choice of $\bbeta$ with the same signs in different components, the norms coincide with classical $\ell_q$ norms even for odd $q$s. We can see $q=2$ has higher power compared to $q=1$ under sparse alternative, which supports our prior that larger $q$ is favored in this case. However, we find that the power decreases as we further increase $q$.

We also repeat the result for $\bbeta=(\bm{1}_{r/2},-\bm{1}_{r/2},\bm{0}_{p-r})$.
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
$(n,p)$ & $\delta,r$ & $q=1$ & $q=2$ & $q=3$ & $q=4$ & $q=5$ & $q=6$ \\ \hline
\multirow{2}{*}{(200, 100)} & 2, 0.3 & 5 & 46 & 28 & 83 & 41 & 74 \\ \cline{2-8}
& $0.1,p$    & 5 & 100 & 24 & 44 & 36 & 21 \\ \hline
\end{tabular}
\caption{Size and power simulation in \%, with variance estimator based on permutation}
\end{table}

In general, if we want to test $\bbeta=\bbeta_0$, we can permute $(X_i,Y_i-X_i^T\bbeta_0)$.



\subsection{Testing Independence}
We consider the following statistics testing component-wise independence.
\begin{itemize}
    \item $U_\tau(q),U_\tau^M(q),U_\tau^I(q)$: $L_q$-type of Kendall's $\tau$ statistic.
    \item $U_\rho(q),U_\rho^M(q),U_\rho^I(q)$: $L_q$-type of Spearman's $\rho$ statistic.
    \item $U_D(q),U_D^M(q),U_D^I(q)$: $L_q$-type of Hoeffding's $D$ statistic.
    \item $U_R(q),U_R^M(q),U_R^I(q)$: $L_q$-type of Blum–Kiefer–Rosenblatt's $R$ statistic.        
    \item $U_{\tau^*}(q),U_{\tau^*}^M(q),U_{\tau^*}^I(q)$: $L_q$-type of Bergsma–Dassios–Yanagimoto’s $\tau^*$ statistic.

    
\end{itemize}
We consider several data generating processes from which we generate i.i.d. data $X_1,\ldots,X_n\in\R^p$.
\paragraph{Settings for Size Simulation}
\begin{itemize}
    \item Standard Gaussian: $X_i\iid N(0,I_p);~i=1,\ldots,n$.
    \item $t$-distribution: $X_{ij}\iid  t_3;~i=1,\ldots,n;j=1,\ldots,p$.
\end{itemize}
We choose $n\in\{100,200\}$, $p\in\{50,100,200,400\}$ We report the size and power based on 1000 Monte Carlo simulations in the following tables.


\begin{table}[H]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
$(n,p)$ & $\delta,r$ & $M$ & Method & $q=1$ & $q=2$ & $q=3$ & $q=4$ & $q=5$ & $q=6$ & $q=2,4$ & $q=2,6$\\ \hline
\multirow{9}{*}{(100,50)} & \multirow{3}{*}{0,NA} & 10 & \multirow{2}{*}{Var-Pmt} & 5 & 9 & 8 & 8 & 5 & 8 & 12 & 11 \\ \cline{3-3} \cline{5-12} 
 &  & \multirow{2}{*}{100} & & 5 & 6 & 4 & 7 & 4 & 7 & 6 & 6\\ \cline{4-12} 
 &  &  & Pval-Pmt & 5 & 4 & 4 & 8 & 5 & 7 & 7 & 9 \\ \cline{2-12} 
 & \multirow{3}{*}{3,0.5} & 10 & \multirow{2}{*}{Var-Pmt} & 18 & 41 & 84 & 96 & 96 & 96 & 94 & 96 \\ \cline{3-3} \cline{5-12} 
 &  & \multirow{2}{*}{100} & & 17 & 35 & 87 & 96 & 97 & 97 & 98 & 96 \\ \cline{4-12} 
 &  &  & Pval-Pmt & 16 & 38 & 88 & 96 & 97 & 96 & 97 & 94 \\ \cline{2-12} 
 & \multirow{3}{*}{$0.05,p$} & 10 & \multirow{2}{*}{Var-Pmt} & 100 & 99 & 44 & 16 & 12 & 9 & 96 & 96\\ \cline{3-3} \cline{5-12} 
 &  & \multirow{2}{*}{100} & & 100 & 99 & 39 & 13 & 10 & 7 & 97 & 97 \\ \cline{4-12} 
 &  &  & Pval-Pmt & 100 & 98 & 42 & 14 & 11 & 8 & 98 & 98
  \\ \hline
\end{tabular}
\end{table}


\paragraph{Settings for Power Simulation}
\begin{enumerate}
    \item Gaussian vectors with banded covariance matrix: $X_i\iid N(0,\Sigma)$ for $i=1,\ldots,n$,
    where $\Sigma=(\sigma_{ab})_{a,b=1}^p$ with $\sigma_{ab}=(1-r)1\{i=j\}+r 1\{i\le h,j\le h\}$.
    \item $t$-distribution with banded covariance matrix: $X_i\iid \Sigma^{1/2}Z$ for $i=1,\ldots,n$, where $\Sigma$ is given above, and $Z_{ij}\iid t_3;~i=1,\ldots,n;j=1,\ldots,p$.
    \item We draw data $X_i\iid N(0,\Sigma)$, with $\Sigma$ being random with eight non-zero off-diagonal terms and constant diagonals. $\Sigma$ is generated by taking four random entries from strict upper triangle, and setting their values to be randomly generated from $Unif(0,1)$. Then we also set four entries from lower triangle to make $\Sigma$ symmetric, and all diagonals to be 1. Finally, if $\Sigma$ we obtained following above approach is not positive definite, with minimal eigenvalue $\delta\le 0$, then we add $\delta+0.5$ to all diagonals of $\Sigma$.
\end{enumerate}
We take $(h,r)\in\{(5,0.9),(p,0.3)\}$ for sparse and dense alternatives.

Take the MDD example we introduced before. Recal we need to simulate the following U-statistic,
\begin{align*}
U_{n,q}=&(P^n_{4q})^{-1}\sum_{l\in\cL}\sum^*_{1\le i_1,\ldots,i_{4q}\le n}\prod_{c=1}^q h_l\big((X_{i_{4c-3}},Y_{i_{(4c-3}}),\ldots,(X_{i_{4c}},Y_{i_{4c}})\big),\\
=&(P^n_{4q})^{-1}\sum_{l\in\cL}\sum^*_{1\le i_1,\ldots,i_{4q}\le n}\prod_{c=1}^q h\big((x_{i_{4c-3},l},Y_{i_{4c-3}}),\ldots,(x_{i_{4c},l},Y_{i_{4c}})\big),
\end{align*}
with $h_l$ given by (\ref{mddkernel}) and (\ref{mdd2}). Then we may approximate its distribution by
$$
U_{n,q}^\sigma=\sum_{l\in\cL}(P^n_{4q})^{-1}\sum^*_{1\le i_1,\ldots,i_{4q}\le n}\prod_{c=1}^q h\big((x_{i_{4c-3},l},Y_{\sigma(i_{4c-3})}),\ldots,(x_{i_{4c},l},Y_{\sigma(i_{4c})})\big),
$$
with random permutation $\sigma$.

-----r=2 proof---
where $\displaystyle\sum_{i_t^{(h)}}^{(1)}$ denotes the summation over terms s.t. the two sets $\big\{i_1^{(1)},i_2^{(1)}\},\ldots,\{i_{2q-3}^{(1)},i_{2q-2}^{(1)}\}\big\}=\big\{\{i_1^{(2)},i_2^{(2)}\},\ldots,\{i_{2q-3}^{(2)},i_{2q-2}^{(2)}\}\big\}$, and $\displaystyle\sum_{i_t^{(h)}}^{(2)}$ is over the other terms. Note that for term has nonzero expectation only if the followings both hold.
\begin{enumerate}
    \item $i_{2q-1}^{(1)}$ coincides with $i_{2q-1}^{(2)}$.
    \item For any $1\le t<q$, $i_t^{(1)}$ matches $i_s^{(2)}$ for some $1\le s<q$. 
\end{enumerate}
Therefore, the summation $\displaystyle\sum_{i_t^{(h)}}^{(2)}$ essentially contains all terms that satisfies the both rules, and at least one $i_{2t-1}^{(1)}$ matches $i_{2s_1-1}^{(1)}$ for some $s_1$ and $i_{2t}^{(1)}$ coincides with $i_{2s_2}^{(2)}$ for some $s_2\not=s_1$  (otherwise the term is included in summation $\displaystyle\sum_{i_t^{(h)}}^{(1)}$).

 When dealing with $\E[h_{l_1}(X_{i_{2q-1}^{(1)}},X_i)h_{l_2}(X_{i_{2q-1}^{(2)}},X_i)|\F_{i-1}]$ term, we can view it as $$\E[h_{l_1}(X_{i_{2q-1}^{(1)}},X_0)h_{l_2}(X_{i_{2q-1}^{(2)}},X_0)|X],$$ where $X_0$ is some non-observed i.i.d. data of observed ones and $X=(X_1,\ldots,X_n)$. Conditional on $X$, we can move other terms inside the conditional expectation and then apply the law of full expectation. Therefore, we can analyze the moment of $V_{1,n}^{(k)}$ equivalently by replacing the conditional expectation $\E[h_{l_1}(X_{i_{2q-1}^{(1)}},X_i)h_{l_2}(X_{i_{2q-1}^{(2)}},X_i)|\F_{i-1}]$ with $h_{l_1}(X_{i_{2q-1}^{(1)}},X_0^{(1)})h_{l_2}(X_{i_{2q-1}^{(2)}},X_0^{(2)})$.

With this trick, straightforward calculation shows that $\E[V_{1,n}^{(1)}]=2^qq!+o(1)$. It remains to show that $\E[(V_{1,n}^{(1)})^2]\rightarrow (2^qq!)^2$ and $\E[(V_{1,n}^{(2)})^2]\rightarrow 0$ which implies $V_{1,n}^{(1)}\cop 2^qq!$ and $V_{1,n}^{(2)}\cop 0$. We can prove the former one similarly to (i) using Lemma \ref{sumcum}, where we take the dummy variables $X_0^{(3)}=X_0^{(4)}$  to be i.i.d. copy of $X_0^{(1)}=X_0^{(2)}$ in the derivation.

For $\E[(V_{1,n}^{(2)})^2]$, note that the leading term has constant order in $n$, and we may apply Assumption \ref{cumrold} A.1 to prove its negligibility as follows. The order satisfies $$\E[(V_{1,n}^{(2)})^2]\lesssim\Sigma^{-2}_2(q)\sum_{l_1,l_2,l_3,l_4\in\cL}\sigma_2^{2d}(l_1,l_2)\sigma_2^{2d}(l_3,l_4)\sigma_2^{2e}(l_1,l_4)\sigma^{2e}(l_2,l_3)\sigma^{2f}_2(l_1,l_3)\sigma_2^{2f}(l_2,l_4),$$ 
with $d>0,e+f>0$ and $d+e+f=q$.  Without loss of generality, we can assume $e>0$. Note that,
\begin{align*}
&\sum_{l_1,l_2,l_3,l_4\in\cL}\sigma_2^{2d}(l_1,l_2)\sigma_2^{2d}(l_3,l_4)\sigma_2^{2e}(l_1,l_4)\sigma_2^{2e}(l_2,l_3)\sigma^{2f}_2(l_1,l_3)\sigma_2^{2f}(l_2,l_4)\\
=&\sum_{l_1,l_2,l_3,l_4\in\cL}[\sigma_2^{2}(l_1,l_2)\sigma_2^{2}(l_3,l_4)\sigma_2^{2}(l_1,l_4)\sigma_2^{2}(l_2,l_3)]\cdot\\
&~~~~~~~~[\sigma_2^{2d-2}(l_1,l_2)\sigma_2^{2d-2}(l_3,l_4)\sigma_2^{2e-2}(l_1,l_4)\sigma_2^{2e-2}(l_2,l_3)\sigma^{2f}_2(l_1,l_3)\sigma_2^{2f}(l_2,l_4)]\\
\le&\left[\sum_{l_1,l_2,l_3,l_4\in\cL}[\sigma_2^{2}(l_1,l_2)\sigma_2^{2}(l_3,l_4)\sigma_2^{2}(l_1,l_4)\sigma_2^{2}(l_2,l_3)]^{q/2}\right]^{2/q}\cdot\\
&\left[\sum_{l_1,l_2,l_3,l_4\in\cL}[\sigma_2^{2}(l_1,l_2)\sigma_2^{2}(l_3,l_4)\sigma_2^{2}(l_1,l_4)\sigma_2^{2}(l_2,l_3)\sigma_2^{2}(l_1,l_3)\sigma_2^{2}(l_2,l_4)]^{q/(q-2)}\right]^{1-2/q}\\
\lesssim&o(\Sigma_2^{4/q}(q))\cdot\Sigma_2^{2(1-2/q)}(q)=o(\Sigma_2^2(q)),
\end{align*}
by Assumption \ref{cumrold} A.1 and Lemma \ref{sumcum}. We can conclude that $\E[(V_{1,n}^{(2)})^2]\rightarrow 0$. 

In conclusion, we have $V_{1,n}\cop(2^qq!)^2$. Similarly we can prove $V_{2,n}\cop(2^QQ!)^2$ and $V_{3,n}\cop0$. Therefore, we have proven (ii).
----

------proof of Lemma (ii)-----------------
We show by induction that for any $1\le c\le q$,
\begin{align*}
&\sum_{l_1,l_2,l_3,l_4\in\cL}\E\left[H_{c,l_1}^{(r)}(X_{i_1^{(1)}},\ldots,X_{i_{cr-1}^{(1)}},X')H_{c,l_2}^{(r)}(X_{i_1^{(2)}},\ldots,X_{i_{cr-1}^{(2)}},X')\right.\\
&~~~~\left.H_{c,l_3}^{(r)}(X_{j_1^{(1)}},\ldots,X_{j_{cr-1}^{(1)}},X'')H_{c,l_4}^{(r)}(X_{j_1^{(2)}},\ldots,X_{j_{cr-1}^{(2)}},X'')\right]\\
=&o(\Sigma_r^{2c/q}(q)).
\end{align*}
For $c=1$, the claim holds as it reduces to the assumption:
\begin{align*}
&\E^{q/c}\left[H_{1,l_1}^{(r)}(X_{i_1^{(1)}},\ldots,X_{i_{r-1}^{(1)}},X')H_{1,l_2}^{(r)}(X_{i_1^{(2)}},\ldots,X_{i_{r-1}^{(2)}},X')\right.\\
&~~~~\left.H_{1,l_3}^{(r)}(X_{j_1^{(1)}},\ldots,X_{j_{r-1}^{(1)}},X'')H_{1,l_4}^{(r)}(X_{j_1^{(2)}},\ldots,X_{j_{r-1}^{(2)}},X'')\right]\\
=& \E\left[h_{l_1}^{(r)}(X_{i_1^{(1)}},\ldots,X_{i_{r-1}^{(1)}},X')h_{l_2}^{(r)}(X_{i_1^{(2)}},\ldots,X_{i_{r-1}^{(2)}},X')\right.\\
&~~~~\left.h_{l_3}^{(r)}(X_{j_1^{(1)}},\ldots,X_{j_{r-1}^{(1)}},X'')h_{l_4}^{(r)}(X_{j_1^{(2)}},\ldots,X_{j_{r-1}^{(2)}},X'')\right]\\
=&\cum\left(h_{l_1}^{(r)}(X_{i_1^{(1)}},\ldots,X_{i_{r-1}^{(1)}},X'),h_{l_2}^{(r)}(X_{i_1^{(2)}},\ldots,X_{i_{r-1}^{(2)}},X'),\right.\\
&~~~~\left.h_{l_3}^{(r)}(X_{j_1^{(1)}},\ldots,X_{j_{r-1}^{(1)}},X''),h_{l_4}^{(r)}(X_{j_1^{(2)}},\ldots,X_{j_{r-1}^{(2)}},X'')\right)=o_p(\Sigma_r^{2/q}(q)),
\end{align*}
where we use the fact that $h_l^{(r)}$ is fully degenerate, and hence any product term of expectation in the cumulant decomposition equals zero.

Suppose the claim holds for $1,\ldots,c-1$. Recall $H_{c,l}^{(r)}$ is the symmetric version of $\otimes^c h_l^{(r)}=\otimes^c h_l$. By H\"{o}lder's inequality, we have
\begin{align*}
&\sum_{l_1,l_2,l_3,l_4\in\cL}\E\left[H_{c,l_1}^{(r)}(X_{i_1^{(1)}},\ldots,X_{i_{cr-1}^{(1)}},X')H_{c,l_2}^{(r)}(X_{i_1^{(2)}},\ldots,X_{i_{cr-1}^{(2)}},X')\right.\\
&~~~~\left.H_{c,l_3}^{(r)}(X_{j_1^{(1)}},\ldots,X_{j_{cr-1}^{(1)}},X'')H_{q,l_4}^{(r)}(X_{j_1^{(2)}},\ldots,X_{j_{cr-1}^{(2)}},X'')\right]\\
\lesssim&\sum_{l_1,l_2,l_3,l_4\in\cL}\E\left[(\otimes ^q h_{l_1})(X_{i_1^{(1)}},\ldots,X_{i_{cr-1}^{(1)}},X')\otimes ^c (h_{l_2})(X_{i_1^{(2)}},\ldots,X_{i_{cr-1}^{(2)}},X')\right.\\
&~~~~\left.\otimes ^c (h_{l_3})(X_{j_1^{(1)}},\ldots,X_{j_{cr-1}^{(1)}},X'')\otimes ^c (h_{l_4})(X_{j_1^{(2)}},\ldots,X_{j_{cr-1}^{(2)}},X'')\right].\\
\end{align*}
---------------------
Omega
We also define $\Omega^{(l_1,\ldots,l_h)}$ as a matrix in $\R^{(p-h)\times (p-h)}$ that drops the $l_1,\ldots,l_h$-th rows and columns of $\Omega$ and 
$$A^{(l_1,\ldots,l_h)}=\left\{ \sum_{l\notin\{l_1,\ldots l_h\}}W_{i,l}^2\ge \frac{\tr(\Omega^{(l_1,\ldots,l_h)})}{2p}\right\}.$$


To check that Assumption \ref{ass::cumr}.1 holds for $Y_i$, note that
\begin{align*}
\|\Sigma_X\|_q^q\deltaeq&\sum_{l_1,l_2=1}^p\cov(x_{1,l_1}\cdots x_{q,l_1},x_{1,l_2}\cdots x_{q,l_2})\\
=&\var\left(\sum_{l=1}^px_{1,l}\cdots x_{q,l}\right)\ge c_0p,
\end{align*}
as the same assumption holds for $X_i$ with $C_p=1$. Therefore, we have
\begin{align*}
\|\Sigma_Y\|_q^q\deltaeq&\var\left(\sum_{l=1}^p\frac{x_{1,l}\cdots x_{q,l}}{\|X_1\|\cdots\|X_q\|}\right)\\
=&\var\left(\sum_{l=1}^p\frac{w_{1,l}\cdots w_{q,l}}{\|W_1\|\cdots\|W_q\|}\right)\\
\ge &\var\left(\sum_{l=1}^p\frac{w_{1,l}\cdots w_{q,l}}{\|W_1\|\cdots\|W_q\|}1_{A_1\cap\cdots\cap 1_{A_q}}\right)
\end{align*}
\begin{align*}
\var(y_{i,l})=&\E\left[\frac{w_{i,l}^2}{\|W_i\|^2}\right]\ge \E\left[\frac{w_{i,l}^2}{\|W_i\|^2}1_{A}\right]\\
\ge&\E\left[\frac{2pw_{i,l}^2}{3\tr(\Omega)}1_{A}\right]=\frac{2P(A)\Omega_{ll}}{3\tr(\Omega)},
\end{align*}
where we have used the definition of the event $A$, and $\E[U_i^2]=p^{-1}I_p$.
Since Assumption \ref{ass::cumr}.1 holds for $X_i$ with $C_p=1$, we have 
$\var(x_{il})=p^{-1}D\Omega_{ll}\ge c_0$, which implies that 
$$
\var(w_{i,l})\ge \frac{2P(A)\Omega_{ll}}{3\tr(\Omega)}\ge c_0'\frac{p}{D\tr(\Omega)},
$$
so Assumption $\ref{ass::cumr}$.1 holds for $\frac{p}{D\tr(\Omega)}$.

